An End-to-End Performance Analysis for Service Chaining in a Virtualized Network

Future mobile networks supporting Internet of Things are expected to provide both high throughput and low latency to user-specific services. One way to overcome this challenge is to adopt Network Function Virtualization (NFV) and Multi-access Edge Computing (MEC). Besides latency constraints, these services may have strict function chaining requirements. The distribution of network functions over different hosts and more flexible routing caused by service function chaining raise new challenges for end-to-end performance analysis. In this paper, as a first step, we analyze an end-to-end communications system that consists of both MEC servers and a server at the core network hosting different types of virtual network functions. We develop a queueing model for the performance analysis of the system consisting of both processing and transmission flows. We propose a method in order to derive analytical expressions of the performance metrics of interest. Then, we show how to apply the similar method to an extended larger system and derive a stochastic model for such systems. We observe that the simulation and analytical results coincide. By evaluating the system under different scenarios, we provide insights for the decision making on traffic flow control and its impact on critical performance metrics.

==> Introduction.tex <==
The increasing demand of different kinds of network services and the requirements of 5G networks for low capital expenditure raise the need for the improvement of today's networks in terms of both flexibility and scalability. In conventional communications networks, network functions (e.g., firewalls, transcoders, load balancers, etc.) are performed as dedicated hardware middleboxes. Although dedicated hardware can provide high performance, it causes high capital expenditure, low flexibility and scalability, and dependence on particular application. In future communications networks, these limitations will be addressed by Network Function Virtualization (NFV)  \cite{NFV_StateOfTheArt, bonfim2018integrated, li2015software}. The idea of NFV is to decouple the network functions from dedicated hardware equipment. More specifically, general purpose servers can host one or more types of network functions. The network can be flexible and it can deploy proper network functions according to the demands of various traffic types while reducing the capital expenditure. Furthermore, mission-critical mobile applications, e.g., augmented reality, connected vehicles, eHealth, will provide services that require ultra-low latency \cite{MECKeyTech}, \cite{taleb2017multi}. To satisfy such requirements, Multi-access Edge Computing (MEC) has been proposed as a key solution \cite{MECKeyTech}. The idea of MEC is to locate more computation resources closer to the users, e.g., at the base stations.
\ac{NFV} together with MEC are considered key technologies for 5G wireless sytems. However, computation capabilities and  available resources of MEC servers are still limited compared to the high-end servers in the cloud. Therefore, it is interesting to further investigate the cooperation between the edge and the core, and the cooperation among MEC servers.
\subsection{Related work}
Recently, the study of the performance of networks in \ac{VNF}/\ac{SDN} environment has  attracted a lot of attention, \cite{YeE2DDelay, duan2018modeling, miao2019stochastic,  lombardo2014analytical,fahmin2017performance,jarschel2011modeling,goto2016queueing,xiong2016performance}.
Ye \etal \cite{YeE2DDelay} analyze the end-to-end delay for embedded VNF chains. They consider two types of services that traverse different \ac{VNF} chains and provide the delay analysis for each different chain.
Miao \etal \cite{miao2019stochastic}  provide an analytical model based on \ac{SNC} to provide upper and lower delay bounds  of a \ac{VNF} chain. In their analysis, they consider both the case of bursty and non-bursty traffic. Along similar lines, Duan \cite{duan2018modeling} analyzes an end-to-end delay performance of service function chaining for particular services and given resources.
Authors in \cite{lombardo2014analytical,fahmin2017performance,jarschel2011modeling, goto2016queueing,xiong2016performance},  apply tools from queueing theory to evaluate the performance of systems in \ac{SDN} environment. In particular, Jarschel  \etal \cite{jarschel2011modeling} study the OpenFlow architecture, where the switch is modeled as an M/M/1 queue and the controller as a feedback system of the delay-loss type M/M/1/S queue. Similarly Goto \etal \cite{goto2016queueing} analyze a simple OpenFlow-based switch in SDN environment, however, they distinguish traffic from the controller and exogenous traffic. 
Furthermore, a reasonable amount of works consider the modeling of connected \acs{VNF} as a sequence of queues where the goal is to guarantee the stability of the system and some particular network or service requirements. A well known and widely used mathematical tool for stabilizing dynamic systems is the Lyapunov optimization theory.
The authors in \cite{feng2018optimal, barcelo2015cloud, feng2016dynamic, feng2018optimalwireless, chen2019automated,gu2019fairness} develop dynamic algorithms by applying Lyapunov optimization theory in order to guarantee system stability and fulfill additional service requirements. In particular, in \cite{feng2018optimal, feng2018optimalwireless} flows traverse \ac{VNF} chains and each node decides the resource allocation to each \ac{VNF} and routes the flow to the next node. Gu \etal \cite{gu2019fairness} develop a dynamic distributed algorithm that controls the flow and rate at each node. Their objective is to achieve fairness between the services and maximize the network utility while providing system stability. Chen \etal \cite{chen2019automated} consider the problem where \ac{VNF} are installed in \acp{VM}. Each  \ac{VM} can be located in the same or different data center. In this work, each \ac{VM} decides which functions to install or uninstall and which services to serve. A dynamic algorithm is developed  that works in a distributed manner and takes online decisions.
Considering a more static and known environment, researchers investigate the \ac{VNF} placement and resource allocation problems \cite{NearOptPlac, JointOptJournal,qu2016delay, xu2019NFVenabled, gouareb2018virtual}. In these works, the authors formulate the VNF placement problem as Mixed Integer Linear Problem (MILP) under the assumption of known traffic demand.  In addition, approximation algorithms have been developed in order to provide a solution to the VNF placement problem, see for example  \cite{feng2017approximation, lange2017multi}. 

Besides the \ac{VNF}/\ac{SDN} technologies, \ac{MEC} technology promises a significant improvement of the networks, especially in terms of latency reduction. Task offloading from the mobile devices to \acp{MEC} has attracted considerable attention. For example, the authors in \cite{liu2016delay, mao2017stochastic, HanPowerOptimalScheduling, lyu2018energy}  address the trade-off between the power consumption and the task processing delay. The authors in \cite{xiangnetworkslicing}, propose an optimization model to perform joint slicing of mobile network and edge computation resources.
As VNF and MEC are two strongly connected technologies, the research evolution of the one affects the evolution of the other. To the best of our knowledge, there are no works providing end-to-end network performance analysis for a network with MEC deployed and operated within the NFV environment.
\subsection{Contributions}
In this paper, we investigate a \ac{VNF}-facilitated end-to-end network where the cooperation between the edge and the core network, and the cooperation among \acp{MEC} are considered. As a first step, we model and analyze a simple end-to-end communications system which consists of two MEC servers at the edge network and one at the core network hosting different types of VNFs. We develop a methodology by applying tools from queueing theory in order to derive approximate analytical expressions of the performance metrics of interest such as end-to-end delay, drop rate, and throughput. The methodology is based on the decomposion of the system into smaller subsystems easier to analyze. The information from analysis of each subsystem can be used in order to study the performance of the entire system. Since, in reality, there are no buffers with infinite capacity, we consider finite size buffers in the servers of our system model. However, the capabilities of the server at the core are considered to be much higher than those of the MEC servers. In order to observe the behavior of the system asymptotically, we also investigate, as a subcase, the scenario where the buffers at  core server is infinite. Based on the methodology derived for the simple model, we extend the analysis to a more complex system with a larger number of MEC servers. As shown in the simulation results, the proposed stochastic model is accurate and indicates a robust behavior even for larger number of servers. Furthermore, we provide results that show the trade-off between the throughput, drop rate, and end-to-end delay. In this work we provide approximate analytical expressions for the  performance metrics of our interest in order to provide  insights of how to design a system to satisfy particular network requirements. 
